More results on stack-sorting for set partitions

Let a sock be an element of an ordered finite alphabet A and a sequence of these elements be a sock sequence. In 2023, Xia introduced a deterministic version of Defant and Kravitz's stack-sorting map by defining the $\phi_{\sigma}$ and $\phi_{\overline{\sigma}}$ pattern-avoidance stack-sorting maps for sock sequences. Xia showed that the $\phi_{aba}$ map is the only one that eventually sorts all set partitions; in this paper, we prove deeper results regarding $\phi_{aba}$ and $\phi_{\overline{aba}}$ as a natural next step. We newly define two algorithms with time complexity $O(n^3)$ that determine if any given sock sequence is in the image of $\phi_{aba}$ or $\phi_{\overline{aba}}$ respectively. We also show that the maximum number of preimages that a sock sequence of length $n$ has grows at least exponentially under both the $\phi_{aba}$ and $\phi_{\overline{aba}}$ maps. Additionally, we prove results regarding fertility numbers (introduced by Defant) in the context of set partitions and multiple-pattern-avoiding stacks.

==> proofs.tex <==
\subsection{Algorithms that characterize the images of $\phi_{\overline{aba}}$ and $\phi_{aba}$}
\begin{proof}[Proof of \Cref{cons_aba_image}]
    We first present the algorithm:
    \begin{enumerate}
    \item Iterate through the sequence, checking if everything to the right of the current sock is already sorted.
    \item If so, denote everything to the left of the current sock as the \textit{left-subsequence} and the rest of the sequence as the \textit{right-subsequence}. Consider the first sock in the left-subsequence. Iterate through the right-subsequence in reverse, looking for two consecutive socks that (a) are the same as each other and (b) are not the same as the first sock in the left-subsequence. Let these socks be denoted as a \textit{consecutive pair}.
    \item  If no such consecutive pair can be found, then go back to (1) and find the next index at which the overall sequence can be split such that the right-subsequence is already sorted.
    \item If such a pair is found, repeat (2) for the next sock in the left-subsequence, searching for two consecutive socks in the right-subsequence that (a) are the same as each other and (b) are not the same as the currently chosen sock in the left-subsequence. However, the search for this consecutive pair must be done by iterating through the right-subsequence in reverse (just as before), with the stipulation that it must begin where we left off previously (i.e. begin with the leftmost sock of the \textit{previous} consecutive pair that was found).
    \item If the end of the left-subsequence is reached (unique consecutive pairs are found for each of them, in reverse order within the right-subsequence), then the given sock sequence is in the image.
    \item If all possible splits of the given sequence have been considered and the end of the left-subsequence has never been reached, the given sock sequence is not in the image.
    \end{enumerate}

    We now show that this algorithm successfully classifies all set partitions, which is made quite evident by \Cref{Lemma2.3}. The algorithm yields a positive result if and only if there exists a split of the sequence such that every sock in the left-subsequence has a corresponding consecutive pair in the right-subsequence, with these corresponding pairs appearing in order from left to right. Thus, a positive result from the algorithm implies we can construct the preimage of the sequence using \Cref{Lemma2.3}: this is done by reversing the right-subsequence and then placing the socks in the left-subsequence in between their corresponding pair in the right-subsequence.

    Next, we show that the algorithm runs in $O(n^3)$ time. Searching for a split such that the right-subsequence is already sorted runs in quadratic time, since iterating through each possible split of the sequence is obviously linear and the process of checking whether the right-subsequence is already sorted is also linear: to do the latter, we simply iterate through from left to right, keeping a list of the socks that have already been seen and ensuring that each sock encountered either has not already been seen or is the same as the one that directly precedes it. 
    
    Subsequently, the creation of a map between socks in the left-subsequence and consecutive pairs in the right-subsequence runs in $O(n)$ time. This process is linear due to the fact that as we iterate through the left-subsequence and search for consecutive pairs in the right-subsequence, we only end up iterating (in reverse) through the right-subsequence once.

    Overall, since these two independent steps of the algorithm run quadratic and linear time, the overall algorithm is cubic in nature.
\end{proof}
\begin{proof}[Proof of \Cref{aba_image}]
We begin by illustrating the algorithm's steps along with two example sock sequences: $\textit{bcbabccdd}$, which \textbf{is} in the image, and $\textit{bcbcbaabcccdd}$, which \textbf{is not} in the image.
\begin{enumerate}
        \item Iterate through the given sequence from left to right until an $aba$ pattern is found. Then, place a \textit{divider} directly before the second appearance of the \textit{a} in the $aba$ pattern that was found. Repeat this process until no $aba$ patterns can be found to the right of the most recently placed divider. For the sake of visualization, these dividers will be denoted with the ``$\|$" symbol. 
        % \item Next, consider the part of the sequence that lies to the right of the divider that was just placed. Iterate through it from left to right until an $aba$ pattern is found. Place another divider directly before the second appearance of the \textit{a} in the \textit{aba} pattern that was found. Repeat this step until no $aba$ patterns can be found to the right of the most-recently-placed divider.
        \item After this procedure, our examples would look as follows:
        \begin{center}
            $\textit{bcbabccdd} \Longrightarrow \textit{bc$\|$ba$\|$bccdd}$\\
            $\textit{bcbcbaabcccdd} \Longrightarrow \textit{bc$\|$bc$\|$baa$\|$bcccdd}$
        \end{center}
    \item Now, we establish a function $\gamma(i)$ that takes in a sock sequence $i$ as input and returns an integer. The algorithm consists of moving from left to right across the sequence and updating $\gamma(i)$. We claim that a sequence $i$ is in the image if and only if $\gamma(i)\geq0$.
    \item The dividers separate the sequence into what we refer to as \textit{blocks}. $\gamma(i)=0$ to start. There are two rules as to how $\gamma(i)$ changes and dividers are manipulated:
    \begin{enumerate}
        \item Every time a divider is encountered, decrease $\gamma(i)$ by one.
        \item As we move from left to right across the sequence, consider the strings of the same sock that appear consecutively. Whenever one such run of the same sock is encountered, $\gamma(i)$ is updated. Consider one such run of socks that has length $l\geq1$ and appears in the $j$-th block of the sequence (counting from the left). Let the repeated sock be denoted $a$. Then, starting from the sock directly preceding $a$ and moving leftwards, consider each sock in the sequence until another $a$ is encountered. Let this first $a$ appear in the $m$-th block, counting from the left; if there are no appearances of $a$, then let $m=0$. Let $k=\min(l-1,j-m-1)$ and increase $\gamma(i)$ by $k$. We finish by manipulating dividers according to the value of $k$: 
        \begin{itemize}
            \item If $k>0$, remove the dividers separating the $(j-k)$-th through the $j$-the block, effectively combining them into one new, larger block.
            \item If $k=0$, neither add nor remove dividers.
            \item If $k=-1$, place a divider directly before the current sock.
        \end{itemize}
    \end{enumerate}

    \item Ultimately, if $\gamma(i)\geq0$ upon the algorithm's completion, the sock sequence $i$ is in the image of the $\phi_{aba}$ map. Contrarily, a negative final value for $\gamma(i)$ indicates that the sock sequence $i$ is not in the image of the $\phi_{aba}$ map.

    \item The below table illustrates the value of $\gamma(i)$ for our two examples at each point where $\gamma(i)$ changes by a nonzero amount. The bolded characters illustrate where we are in the sequence at a particular step (note that if a sock that directly follows a divider is bolded, it means that one was just subtracted from $\gamma(i)$ due to the divider's presence).

    \begin{center}
    \begin{tabular}{ c | c | c | c }
    \hline
    Sequence & $\gamma(i)$ & Sequence & $\gamma(i)$ \\
    \hline
     \textit{\textbf{b}c$\|$ba$\|$bccdd} & 0 & \textit{\textbf{b}c$\|$bc$\|$baa$\|$bcccdd} & 0\\ 
     \textit{bc$\|$\textbf{b}a$\|$bccdd} & -1 & \textit{bc$\|$\textbf{b}c$\|$baa$\|$bcccdd} & -1\\ 
     \textit{bc$\|$ba$\|$\textbf{b}ccdd} & -2 & \textit{bc$\|$bc$\|$\textbf{b}aa$\|$bcccdd} & -2\\ 
     \textit{bc$\|$babc\textbf{c}dd} & -1 & \textit{bc$\|$bcba\textbf{a}$\|$bcccdd} & -1\\  
     \textit{bcbabccd\textbf{d}} & \boxed{0} & \textit{bc$\|$bcbaa$\|$\textbf{b}cccdd} & -2\\   
     & & \textit{bc$\|$bcbaa$\|$bcc\textbf{c}dd} & -2\\  
     & & \textit{bc$\|$bcbaabcccd\textbf{d}} & \boxed{-1}\\  
    \end{tabular}
    \end{center}
\end{enumerate}

We now show that this algorithm successfully classifies all set partitions, which is made easier by \Cref{Xialemma2.1}.
The initial assignment of dividers splits up the sequence into the least number of blocks such that each block is already sorted (i.e. does not contain any patterns that are order-isomorphic to $aba$). It is obvious from \Cref{Xialemma2.1} that any sorted sock sequence is in the image of $\phi_{aba}$. Essentially, the algorithm attempts to combine these initial blocks (by removing dividers) into longer and longer sequences that are also in the image of $\phi_{aba}$.

If $p$ blocks $r_1, r_2,\ldots,r_p$ appear in that order, then the definition of dividers implies that $r_1,r_2,\ldots,r_p\in \text{img}(\phi_{aba})$ but $r_1r_2\ldots r_{p-1} \notin \text{img}(\phi_{aba})$. The recursive nature of \Cref{Xialemma2.1} tells us that combining $r_1,r_2,\ldots, r_{p-1}$ whilst ensuring that the result is in the image of $\phi_{aba}$ must use $p-1$ consecutive copies of the same sock $x$, which we will refer to as the \textit{splitting block}. \Cref{Xialemma2.1} requires that the sock $x$ must not be found in $r_1,r_2,\ldots r_{p-1}$; note that it is impossible for $x$ to appear at the end of $r_{p-1}$ while $r_p$ begins with $x^{p-1}$ since dividers will never separate two copies of the same sock due to the manner in which they are assigned. Applying \Cref{Xialemma2.1} with this setup shows that $r_1r_2\ldots r_{p-1}x^{p-1}$ has $\Pi_{k=1}^pxr_k$ as its preimage and thus must be in the image of $\phi_{aba}$. So, we combine the blocks $r_1, r_2,\ldots,r_p$ (removing $p-1$ dividers in the process). However, when any $p$ blocks $r_1, r_2,\ldots,r_p$ are combined according to the algorithm, the combined sequence $r_1 r_2\ldots r_{p-1}r_p$ is not yet confirmed to be in $\text{img}(\phi_{aba})$ until the algorithm has passed completely through the end of $r_p$. Consider the sock $y$ appearing after the splitting block in $r_p$ that also appears in one of $r_1,r_2,\ldots,r_{p-1}$. By \Cref{Xialemma2.1}, $r_1 r_2\ldots r_{p-1}r_p$ cannot be in $\text{img}(\phi_{aba})$; we handle this scenario with the $k=-1$ case of step 5b: a divider is added directly before the sock $y$ and now the block directly preceding this divider (which contains the original $r_1,r_2,\ldots,r_{p-1}$, and part of the original $r_p$) is in $\text{img}(\phi_{aba})$.

Thus, once the algorithm completes, all of the blocks that constitute the sequence must be in $\text{img}(\phi_{aba})$. So, if no dividers remain ($\gamma(i)\geq0$), then we have proven that the entire sequence is in $\text{img}(\phi_{aba})$. 

To prove that $\gamma(i)<0$ implies that the sequence is not in $\text{img}(\phi_{aba})$, we notice that the algorithm maximizes the number of dividers removed by considering every possible splitting block as it passes through the sequence. The theoretical maximum for the number of dividers removed would simply be the sum of the lengths (minus one) of each consecutive string of socks (i.e. $(1-1)+(3-1)+(2-1)=3$ for $abbbcc$). The algorithm cannot attain this maximum when the socks in the splitting block also appear in a previous block, which is handled in step 5: we simply remove the maximum number of dividers such that the combined block does not contain non-consecutive copies of the sock in the splitting block.

Finally, we show that the time complexity of the algorithm is $O(n^3)$. The initial assignment of dividers is a linear process: we keep track of the already-seen socks as we move through the sequence, and every time a pattern isomorphic to $aba$ is discovered, a divider is placed and we begin iterating immediately after the divider.

The rest of the algorithm consists of examining consecutive strings of the same sock $a$. Finding these strings is clearly a linear process (we keep track of the most-recently seen sock as we iterate through the sequence). Once each string is found, we iterate in reverse from the beginning of the string to the beginning of the entire sequence, looking for another appearance of $a$ in a preceding block that will eventually determine the value of $k$ (to compute this, we also keep track of where dividers are placed at any given time in order to count blocks easily)—this is also a linear process.

Thus, the procedures described in steps 4 and 5 run in quadratic time. Combining this with the fact that the initial assignment of dividers is a linear process, the entire algorithm therefore runs in cubic time.
\end{proof}


\subsection{On the preimages and fertility numbers of $\phi_{\overline{aba}}$ and $\phi_{aba}$}

\begin{proof}[Proof of \Cref{pconsimg_exp}]
     Consider the sock sequence $p^* = a_1a_2\cdots a_n a_{n+1}^{k}$ with length $l$. We construct one of its preimages $p$, which clearly must be a sock sequence of length $k+n$.
    The first sock of $p$ must be $a_{n+1}$. Now consider the $k+n-1$ remaining spots of $p$. We choose $k-1$ of these spots for the remaining copies of $a_{n+1}$. Since there is only one copy of each of $a_1,a_2,\cdots,a_{n}$and $(k+n-1)-(k-1)=n$ spots remaining in $p$, the rest of the construction is forced by \Cref{cons_aba_image}.
    To see why, let $j\leq n$ denote the number of unoccupied spots in $p$ that occur before the final copy of $a_{n+1}$. By \Cref{cons_aba_image}, these spots must be filled by $a_1,a_2,\cdots, a_{j}$ in that order from left to right. Then, \Cref{cons_aba_image} also dictates that $p$ must end with the string $a_na_{n-1}a_{n-2}\ldots a_{j+1}$ (as there must necessarily exist $n-j$ unoccupied spots in $p$ that occur consecutively after the last copy of $a_{n-1}$). 
    Thus, there are exactly $\binom{k+n-1}{k-1}$ preimages of $p^*$. Then, setting $n=k=\frac{l}{2}$ results in $\binom{l-1}{\frac{l}{2}-1}$ preimages. Through Stirling's approximation, $\binom{l-1}{\frac{l}{2}-1} \approx \frac{2^n}{\sqrt{2\pi n}}$ so the maximum number of preimages of a sock sequence of length $n$ under the $\phi_{\overline{aba}}$ map grows at least exponentially with $n$. 
\end{proof}

We use a similar technique to prove the same result for $\phi_{aba}$.

\begin{proof}[Proof of \Cref{pimg_exp}]
    Consider the sock sequence $p^*=a_1a_2\cdots a_n a_{n+1}^k$ with length $l$. We construct one of its preimages $p$, which clearly must be a sock sequence of length $k+n$.
    Firstly, note that $p$ must start with $a_{n+1}$ by \Cref{Xialemma2.1}. Now consider the $k+n-1$ remaining spots of $p$. We choose $k-1$ of these spots for the remaining copies of $a_{n+1}$. Since there is only one copy of each of $a_1,a_2,\cdots,a_{n}$and $(k+n-1)-(k-1)=n$ spots remaining in $p$, the rest of the construction is forced by \Cref{Xialemma2.1}: the non-occupied spots must be filled by $a_n,a_{n-1},\cdots,a_{1}$ in that order from left to right. Thus, there are exactly $\binom{k+n-1}{k-1}$ preimages of $p^*$. Then, setting $n=k=\frac{l}{2}$ results in $\binom{l-1}{\frac{l}{2}-1}$ preimages. Again by Stirling's approximation, $\binom{l-1}{\frac{l}{2}-1} \approx \frac{2^n}{\sqrt{2\pi n}}$ so the maximum number of preimages of a sock sequence of length $n$ under the $\phi_{aba}$ map also grows at least exponentially with $n$. 
\end{proof}

\begin{proof}[Proof of \Cref{fert_aba_cons}]
    Specifically, we show that $q=a_1{a_2}^ma_3a_4\ldots a_{n-m+1}$, a sock sequence of length $n$, has $m$ preimages, where $m,n\in \mathbb{Z}$, $m\leq n-1$, and $a_k$ and $a_j$ denote distinct socks if and only if $k\neq j$.
    
    To see this, consider all sock sequences that have the same distribution of socks (up to equivalence) as the final sock sequence $a_1{a_2}^ma_3a_4\ldots a_{n-m+1}$. Clearly, inputs without this property don't map to the desired sock sequence.
    
    It is impossible for $a_2$ to be in the sandwich set of $q$, since there is only one copy of each of the socks $a_1, a_3, a_4,\ldots a_{n-m+1}$. Then, by \Cref{Lemma2.3}, any preimage of $q$ must have either an empty sandwich set or $a_1$ as the only member of its sandwich set. Essentially, any preimage of $q$ must begin with $a_{n-f+1}a_{n-f}\ldots a_4a_3a_2$. 
    
    Then, the remainder of the input sequence must be some rearrangement of $a_1$ and $m-1$ copies of $a_2$. Thus, the sock sequence $q=a_1{a_2}^ma_3a_4\ldots a_{n-m+1}$ has $m$ preimages.
\end{proof}

\begin{proof}[Proof of \Cref{fert_aba}]
    Specifically, we show that $q=a_1a_2a_3\ldots a_{m-1}a_{m}a_ma_{m+1}a_{m+2}\ldots a_{n-2}a_{n-1}$, a sock sequence sock sequence of length $n$, has $m$ pre-images, where $m,n\in \mathbb{Z}$, $m\leq n-1$, and $a_k$ and $a_j$ denote distinct socks if and only if $k\neq j$.

    To see this, consider all sock sequences that have the same distribution of socks (up to equivalence) as the desired sock sequence $a_1a_2a_3\ldots a_{m-1}a_{m}a_ma_{m+1}a_{m+2}\ldots a_{n-2}a_{n-1}$. Clearly, inputs without this property don't map to the desired sock sequence and thus are not preimages of $p$.

    By \Cref{Xialemma2.1}, the string of socks $a_{n-1}\ldots a_{m+1}a_m$ must appear at the beginning of any preimage of $q$, in that order. Then, let $k$ equal \textit{one more than} the number of socks strictly between the first and second appearances of $a_m$; clearly, $k\leq m$. \Cref{Xialemma2.1} dictates that the string of socks $a_{k-1}a_{k-2}\ldots a_2a_1$ must appear, in that order, between the two appearances of $a_m$. Moreover, by \Cref{Xialemma2.1}, any preimage of $q$ must conclude with the string of socks $a_{m-1}a_{m-2}\ldots a_{k+1}a_k$.
    There are thus $m$ spots for the second appearance of $a_m$, as $k$ ranges from 1 to $m$ inclusive. Thus, since each value of $k$ corresponds to exactly one preimage, the sock sequence $q=a_1a_2a_3\ldots a_{m-1}a_{m}a_ma_{m+1}a_{m+2}\ldots a_{n-2}a_{n-1}$ has $m$ preimages.
\end{proof}

\subsection{Results regarding multiple-pattern-avoidance stack-sorting maps}
\begin{proof}[Proof of \Cref{multpat}]
    We consider two cases.\\
    \underline{Case 1:} Either all elements of $G$ contain a pattern order-isomorphic to $abba$ or $abca$, or all do not. By applying \Cref{Xiaproposition2.2}, we can evidently construct a sequence $p$ that is never sorted by the stack.\\
    \underline{Case 2:} $G$ has elements that contain patterns order-isomorphic $abba$ or $abca$ as well as elements that contain patterns order-isomorphic to $abab$, $abac$, or $caba$. In this case, consider the sequence $p=a_1a_2a_1a_3a_1a_4\cdots a_1a_ma_1$, where there is a new distinct sock between every pair of $a_1$s. As this sequence passes through the stack, it becomes $p^*=a_1a_3a_1a_4a\cdots a_1a_ma_1a_2a_1$, which is equivalent to the original sequence $p$, so $p$ will never be sorted.  
\end{proof}

\begin{proof}[Proof of \Cref{gnrfct}]
    We consider two cases.\\
    \underline{Case 1:} Either all elements of $G$ contain a pattern order-isomorphic to $abba$ or $abca$, or all do not. By applying \Cref{Xiaproposition2.2}, we can evidently construct a sequence $p$ that is never sorted by the stack.\\
    \underline{Case 2:} $G$ has elements that contain patterns order-isomorphic $abba$ or $abca$ as well as elements that contain patterns order-isomorphic to $abab$, $abac$, or $caba$. In this case, consider the sequence $p=a_1a_2a_1a_3a_1a_4\cdots a_1a_ma_1$, where there is a new distinct sock between every pair of $a_1$s. As this sequence passes through the stack, it becomes $p^*=a_1a_3a_1a_4a\cdots a_1a_ma_1a_2a_1$, which is equivalent to the original sequence $p$, so $p$ will never be sorted.  
\end{proof}


